PipeInfer: Accelerating LLM Inference using Asynchronous Pipelined Speculation

Inference of Large Language Models (LLMs) across computer clusters has become a focal point of research in recent times, with many acceleration techniques taking inspiration from CPU speculative execution. These techniques reduce bottlenecks associated with memory bandwidth, but also increase end-to-end latency per inference run, requiring high speculation acceptance rates to improve performance. Combined with a variable rate of acceptance across tasks, speculative inference techniques can result in reduced performance. Additionally, pipeline-parallel designs require many user requests to maintain maximum utilization. As a remedy, we propose PipeInfer, a pipelined speculative acceleration technique to reduce inter-token latency and improve system utilization for single-request scenarios while also improving tolerance to low speculation acceptance rates and low-bandwidth interconnects. PipeInfer exhibits up to a 2.15$\times$ improvement in generation speed over standard speculative inference. PipeInfer achieves its improvement through Continuous Asynchronous Speculation and Early Inference Cancellation, the former improving latency and generation speed by running single-token inference simultaneously with several speculative runs, while the latter improves speed and latency by skipping the computation of invalidated runs, even in the middle of inference.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> sections/figtex/f07_speed_low_perf_cluster.tex <==
\begin{figure}
\includegraphics[width=0.7\linewidth]{sections/figtex/figures/speeds-weak-cluster.pdf}

  \caption{Generation speeds of model pairs using small speculative models on constrained clusters.
  }
  \label{fig:low-spec-speeds}
\end{figure}

==> sections/figtex/f10_memory_efficiency.tex <==
\begin{figure*}
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{subfigure}{.33\linewidth}
        \centering
        \includegraphics[width=\textwidth]{sections/figtex/figures/mem-dolphin-small.pdf}
        \caption{Dolphin-70B paired with TinyLlama-1.1B.}
    \end{subfigure}
    \begin{subfigure}{.33\linewidth}
        \centering
        \includegraphics[width=\textwidth]{sections/figtex/figures/mem-goliath-small.pdf}
        \caption{Goliath-120B paired with XWin-7B.}
    \end{subfigure}
    \begin{subfigure}{.33\linewidth}
        \centering
        \includegraphics[width=\textwidth]{sections/figtex/figures/mem-falcon-small.pdf}
        \caption{Falcon-180B paired with Falcon-7B.}
    \end{subfigure}
  }

  \caption{Memory efficiency of model pairs using small speculative models.
  }
  \label{fig:ram-efficiency}



\end{figure*}

==> sections/figtex/fig-speeds-dolphin.tex <==
\begin{figure}
    \includegraphics[width=\linewidth]{sections/figtex/figures/speeds-dolphin.pdf}
    \caption{Dolphin-70B speeds using different speculative models.}
    \label{fig:dolphin-speeds-nova}

\end{figure}

==> sections/figtex/fig-speeds-falcon.tex <==
\begin{figure}
    \includegraphics[width=\columnwidth]{sections/figtex/figures/speeds-falcon.pdf}
    \caption{Falcon-180B speeds using Falcon-7B or Falcon-40B speculative models.}
    \label{fig:falcon-speeds-nova}

\end{figure}

==> sections/figtex/fig-speeds-goliath.tex <==
\begin{figure}
    \includegraphics[width=\columnwidth]{sections/figtex/figures/speeds-goliath.pdf}
    \caption{Goliath-120 speeds using XWinLM-7B or XWinLM-13B speculative models.}
    \label{fig:goliath-speeds-nova}

\end{figure}

==> sections/figtex/fr08_ttft_latency.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{sections/figtex/figures/ttft-weak.pdf}
    \caption{Time to First Token Latency (TTFT) under different inference methods and models on 4-node Xeon E5 cluster.}
    \label{fig:ttft-latency-low-spec}
\end{figure}

==> sections/figtex/itl-nova.tex <==
\begin{figure}
\centering
    \includegraphics[width=0.75\columnwidth]{sections/figtex/figures/itl-dolphin.pdf}
    \caption{Dolphin-70B paired with TinyLlama/Orca2.}
    \label{fig:itl-dolphin}


\end{figure}

\begin{figure}
\centering
    \includegraphics[width=0.75\columnwidth]{sections/figtex/figures/itl-goliath.pdf}
    \caption{Goliath-120B paired with XWin-7B/13B.}
    \label{fig:itl-goliath}



\end{figure}

\begin{figure}
\centering
    \includegraphics[width=0.75\columnwidth]{sections/figtex/figures/itl-falcon.pdf}
    \caption{Falcon-180B paired with Falcon-7B/40B.}
    \label{fig:itl-falcon}

\end{figure}

% \begin{figure}
%     \includegraphics[width=\columnwidth]{sections/figtex/figures/itl-all.pdf}
%     \caption{Falcon-180B paired with Falcon-7B/40B.}

% \end{figure}

==> sections/figtex/mem-efficiency.tex <==
\begin{figure}
    \includegraphics[width=0.7\columnwidth]{sections/figtex/figures/mem-efficiency.pdf}
    \caption{Memory Efficiency. The Y axis is in logarithmic scale.}
    \label{fig:ram-efficiency}

\end{figure}

==> sections/figtex/speeds_nova.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{sections/figtex/figures/speeds-dolphin.pdf}
    \caption{Dolphin-70B speeds using TinyLlama or Orca2 speculative models.}
    \label{fig:dolphin-speeds-nova}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{sections/figtex/figures/speeds-goliath.pdf}
    \caption{Goliath-120 speeds using XWinLM-7B or XWinLM-13B speculative models.}
    \label{fig:goliath-speeds-nova}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.9\columnwidth]{sections/figtex/figures/speeds-falcon.pdf}
    \caption{Falcon-180B speeds using Falcon-7B or Falcon-40B speculative models.}
    \label{fig:falcon-speeds-nova}
\end{figure}

==> sections/figtex/ttft_nova.tex <==
\begin{figure}
\centering
    \includegraphics[width=0.9\columnwidth,trim={0 0 4cm 0},clip]{sections/figtex/figures/ttft-dolphin.pdf}
    \caption{Dolphin-70B paired with TinyLlama/Orca2.}
    \label{fig:ttft-dolphin}
\end{figure}

\begin{figure}
\centering
    \includegraphics[width=0.9\columnwidth]{sections/figtex/figures/ttft-goliath.pdf}
    \caption{Goliath-120B paired with XWin-7B/13B.}
     \label{fig:ttft-goliath}

\end{figure}

\begin{figure}
\centering
    \includegraphics[width=0.9\columnwidth]{sections/figtex/figures/ttft-falcon.pdf}
    \caption{Falcon-180B paired with Falcon-7B/40B.}
     \label{fig:ttft-falcon}

\end{figure}

==> sections/table/t03_gen_speed.tex <==
\begin{table*}
    
\begin{center}
\caption{Generation Speed (tokens / second)}
\label{tab:g_speed}
\begin{tabular}{ c | c | c | c | c | c }
% \hline
 % \multicolumn{4}{|c|}{Generation Speed (tokens / second)} \\
 % \hline
 \toprule
 Cluster & Model Pair & Iterative Inference & Speculative Inference & PipeInfer & Speedup over Speculation\\ 
 \toprule
 1 Node Xeon & Dolphin & 0.94 & N/A & N/A & N/A \\
 1 Node Xeon & Goliath & 0.53 & N/A & N/A & N/A \\
 1 Node Xeon & Falcon & 0.39 & N/A & N/A & N/A \\
 3 Node EPYC & Falcon & 4.15 & 3.635 & 3.721 & 1.02x\\
 4 Node Xeon & Dolphin & 1.20 & 1.255 & 1.275 & 1.01x\\
 4 Node Xeon & Goliath & 0.30 & 0.542 & 0.65 & 1.19x\\
 4 Node Xeon & Falcon & 0.52 & 0.558 & 0.627 & 1.12x\\
 8 Node Xeon & Dolphin & 0.71 & 0.904 & 1.398 & 1.54x\\  
 8 Node Xeon & Goliath & 0.33 & 0.399 & 0.707 & 1.77x \\
 8 Node Xeon & Falcon & 0.38 & 0.422 & 0.837 & 1.98x\\
 13 Hetero. Nodes & Dolphin & 0.65 & 0.773 & 1.319 & 1.70x\\
 13 Hetero. Nodes & Goliath & 0.349 & 0.395 & 0.850 & 2.15x\\
 13 Hetero. Nodes & Falcon & 0.15 & 0.163 & 0.312 & 1.91x\\
  \toprule

\end{tabular}
\end{center}
\end{table*}

==> sections/table/t04_ram.tex <==
\begin{table*}
    
\begin{center}
\caption{RAM Usage Per Node (GB)}
\label{tab:g_speed}
\begin{tabular}{ c | c | c | c | c | c }
% \hline
 % \multicolumn{4}{|c|}{Generation Speed (tokens / second)} \\
 % \hline
 \toprule
 Cluster & Model Pair & Single-Node Inference & Pipeline-Parallel Naive Inference & Pipeline-Parallel Speculation (Target) & PipeInfer (Target)\\ 
 \toprule

 8 Node Xeon & Dolphin & 32.0 & 3.9 & 4.68 & 4.68 \\  
 8 Node Xeon & Goliath & 47.8 & 6.4 & 8.0 & 8.0 \\
 8 Node Xeon & Falcon & 70.2 & 6.76 &  10 & 10 \\
  \toprule

\end{tabular}
\end{center}
\end{table*}

==> sections/table/t05_latency.tex <==
\begin{table*}
    
\begin{center}
\caption{Generation Latencies (s)}
\label{tab:g_speed}
\begin{tabular}{ c | c | c | c | c | c | c }
% \hline
 % \multicolumn{4}{|c|}{Generation Speed (tokens / second)} \\
 % \hline
 \toprule
  & \multicolumn{2}{c|}{Iterative Inference} & \multicolumn{2}{c|}{Speculative Inference} & \multicolumn{2}{c}{PipeInfer}\\ 
 \toprule
 Model Pair & Time to First Token & Inter-Token Latency & Time to First Token & Inter-Token Latency & Time to First Token & Inter-Token Latency \\
 \toprule
 Dolphin & 1.17 & 0.83 & 4.59 & 0.80 & 1.039 & 0.788\\
 Goliath & 1.56 & 1.54 & 4.826 & 1.72 & 1.653 & 1.661\\
 Falcon & 2.41 & 2.385 & 5.54 & 1.77 & 2.04 & 1.59\\
  \toprule

\end{tabular}
\end{center}
\end{table*}
